Hierarchical Flow Diffusion for Efficient Frame Interpolation

Most recent diffusion-based methods still show a large gap compared to non-diffusion methods for video frame interpolation, in both accuracy and efficiency. Most of them formulate the problem as a denoising procedure in latent space directly, which is less effective caused by the large latent space. We propose to model bilateral optical flow explicitly by hierarchical diffusion models, which has much smaller search space in the denoising procedure. Based on the flow diffusion model, we then use a flow-guided images synthesizer to produce the final result. We train the flow diffusion model and the image synthesizer end to end. Our method achieves state of the art in accuracy, and 10+ times faster than other diffusion-based methods. The project page is at: https://hfd-interpolation.github.io.

==> tables/ablation_study.tex <==
\begin{tabular}{l|cc|cc}
     \toprule
    \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    \multicolumn{5}{c}{\#1 Condition Representation}\\
    Pixel            & 0.0430             & 17.197       & 0.0902         & 30.483     \\
    VQ-GAN           & 0.0424             & 16.924       & 0.0893         & 29.941                 \\
    \bf{Ours}        & {\bf 0.0418}       & {\bf 16.453} & {\bf 0.0870}   & {\bf 29.454}   \\
    \midrule
    \multicolumn{5}{c}{\#2 Target Representation}\\
    Pixel           & 0.0442            & 19.674            &   0.0956      & 39.642              \\
    \bf{Flow}       & \bf{0.0405}       & \bf{15.320}        & \bf{0.0842}   & \bf{27.356} \\
    \midrule
    \multicolumn{5}{c}{\#3 Progressive Training}\\
    Flow loss       &  0.0416            & 16.158             & 0.0865        & 28.767     \\
    % + Image loss    &  0.0411            & 16.093             & 0.0854        & 27.946      \\
    + Image loss & \bf{0.0405}       & \bf{15.320}        & \bf{0.0842}   & \bf{27.356} \\
    \midrule
    \multicolumn{5}{c}{\#4 Optimization Strategy}\\
    Seperate        & 0.0418            & 16.324             & 0.0870        &  29.913             \\
    % Recu rrent       & 0.0409            &  15.782            & 0.0853        &  27.892             \\
    \bf{Joint}      & \bf{0.0405}       & \bf{15.320}        & \bf{0.0842}   & \bf{27.356} \\
    \bottomrule
    %  \multicolumn{5}{c}{\#5 Input Resolution}\\
    % 128                 & 0.0427        & 16.737            & 0.0887            & 29.774              \\
    % 256                 & 0.0405        & 15.320            & 0.0842            & 27.356 \\
    % 512                 & \bf{0.0397}   & \bf{15.026}       & \bf{0.0836}       & \bf{26.925}          \\
    % \bottomrule
\end{tabular}

==> tables/compare_condition.tex <==
\begin{tabular}{l|cc|cc}
     \toprule
    \multirow{2}{*}{Condition}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    Pixel            & 0.0430             & 17.197       & 0.0902         & 30.483     \\
    VQ-GAN           & 0.0424             & 16.924       & 0.0893         & 29.941                 \\
    \bf{Ours}        & {\bf 0.0418}       & {\bf 16.453} & {\bf 0.0870}   & {\bf 29.454}   \\
    \bottomrule
\end{tabular}

==> tables/compare_diffuse_steps.tex <==
\begin{tabular}{cc|cc|cc}
     \toprule
    \multirow{2}{*}{steps}  & \multirow{2}{*}{schedule } & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & ~     & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    1               &  [0, 1]              &                   &               &                      \\
    4               &  [2, 2]              &                   &               &                       \\
    8               &  [2, 6]              &                   &               &                       \\
    8               &  [4, 4]              &                   &               &                       \\
    8               &  [6, 2]              &                   &               &                       \\
    16              &  [8, 8]             &                   &               &                           \\
    \bottomrule
\end{tabular}

==> tables/compare_diffusion_scale.tex <==
\begin{tabular}{ll|ll|ll}
    \toprule
    \multirow{2}{*}{scale} & \multirow{2}{*}{steps} & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                       & ~                     & LPIPS  & FID                      & LPIPS & FID  \\
    \midrule
    % 1/4         & 192   &       &       &       &       \\
    4         & 12                  & 0.0418      & 16.435      &0.0870       & 29.454       \\
    % 1/4         & 384   &       &       &       &        \\
    8         & 12                  & 0.0427      & 16.736      & 0.0886      &  29.796      \\
    16        & 12    &       &           &           &       \\
    \midrule
    % 1/8        & 256   &       &       &       &        \\
    % 1/4 + 1/8   & 192      &       &       &        &         \\ 
    4, 8   &    6, 6   &       &       &        &         \\ 
    4, 8, 16  &    4, 4, 4   &       &       &        &         \\ 
    4, 8, 16, 32 &    3, 3, 3, 3   &       &       &        &         \\ 
    \bottomrule 
\end{tabular}

==> tables/compare_diffusion_space.tex <==
\begin{tabular}{c|cc|cc}
     \toprule
    \multirow{2}{*}{condition}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    Image            & 0.043             & 17.197       & 0.090         & 30.483     \\
    VQ-GAN           & 0.042             & 16.924       & 0.089         & 29.941                 \\
    \bf{Ours}        & {\bf 0.042}       & {\bf 16.393} & {\bf 0.087}   & {\bf 29.927}   \\
    \bottomrule
\end{tabular}

% \begin{tabular}{c|cc|cc}
%      \toprule
%     condition       & LPIPS(h)          & FID(h)               & LPIPS(e)         & FID(e)                   \\
%     \midrule
%     Image            &                   &               &                      \\
%     VQ-GAN           &                   &              &                           \\
%     Ours-1/4         &                   &              &                           \\
%     \bottomrule
% \end{tabular}

==> tables/compare_flow_image.tex <==
\begin{tabular}{c|cc|cc}
     \toprule
    \multirow{2}{*}{target}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    image           &           &           &       &       \\
    flow             &          &           &       &       \\
    \bottomrule
\end{tabular}

==> tables/compare_optimize_diffusion.tex <==
\begin{tabular}{c|cc|cc}
     \toprule
    \multirow{2}{*}{} & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                      & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    separate              &                &                   &               &                      \\
    recurrent           &                &                   &               &                       \\
    joint               &                &                   &               &                       \\
    \bottomrule
\end{tabular}

==> tables/compare_other_psnr_ssim.tex <==
\begin{tabular}{l|cc|cc}
    \toprule
     \multirow{2}{*}{Method}    & \multicolumn{2}{c|}{DAVIS}       & \multicolumn{2}{c}{Vimeo-90k} \\
     ~                          & PSNR     & SSIM                   & PSNR     & SSIM           \\
     \midrule
     VFIformer          & 26.241     & 0.850            &  36.503       & 0.982        \\
     EMA-VFI            & 27.111    & 0.871              & 36.642     & 0.982 \\
     AMT-G              & 27.234     & 0.877            & 36.530         & 0.982  \\
     LDMVFI             & 25.073    & 0.819            &  33.089        & 0.963\\
     MADIFF             & 26.069     & 0.853            &  -    &    -     \\
     Per-VFI            & 26.454     & 0.864             & 33.716        & 0.966    \\
     CBBD               & 26.385     & 0.857            & 35.398           & 0.977       \\
     
     \textbf{Ours}      & 26.870        & 0.866           & 35.641          &0.977              \\
     \bottomrule
     
\end{tabular}

==> tables/compare_prediction.tex <==
\begin{tabular}{lcc|cc}
     \toprule
    \multirow{2}{*}{Target}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    Latent           & 0.0442            & 19.674            &   0.0956      & 39.642              \\
    \bf{Flow}       & \bf{0.0405}       & \bf{15.320}        & \bf{0.0842}   & \bf{27.356} \\
    \bottomrule
\end{tabular}

==> tables/compare_snufilm_psnr_ssim.tex <==

\begin{tabular}{l|cc|cc|cc|cc}
    \toprule
     \multirow{2}{*}{Method} & \multicolumn{2}{c|}{easy} & \multicolumn{2}{c|}{medium} & \multicolumn{2}{c|}{hard}  & \multicolumn{2}{c}{extreme}\\
     ~                              & PSNR          & SSIM           & PSNR      & SSIM             & PSNR          & SSIM           & PSNR     & SSIM       \\
     \midrule
     AMT-G                          & 39.880        & 0.991         & 36.120        & 0.981         & 30.780         & 0.939        & 25.430     & 0.865    \\
     SGM-VFI                        & 40.347       & 0.991        & 36.198        & 0.980              & 30.745            & 0.936        & 25.468           & 0.863          \\
     EMA-VFI                        & 39.520       & 0.990         & 35.830        & 0.979         & 30.790            & 0.939        & 25.590     & 0.865    \\
     URPNet-Large                   & 40.440        & 0.991         & 36.290        & 0.980         & 30.860            & 0.938        & 25.630     & 0.864   \\
     LDMVFI                         & 38.674       & 0.983         & 33.996        & 0.970         & 28.547            & 0.917        & 23.934     & 0.837    \\
     MADIFF                         & 38.644       & 0.988         & 34.255        & 0.973         & 28.961            & 0.923         & 24.150     & 0.847   \\
     % FILM~\cite{reda2022film}        & 0.0120    &               & 0.0213       &           & 0.0429        &           & 0.0889        &       \\
     CBBD                           & 39.637       & 0.990         & 34.886        & 0.974         & 29.615            & 0.929        & 24.376     & 0.848    \\
    %eMOMO~\cite{lew2024disentangled} & 0.011    &                  & 0.020     &         & 0.042     &              & 0.087 & \\
     \textbf{Ours}                   & 39.743   & 0.987    & 35.694        & 0.975         & 30.375            & 0.931        & 25.163         &0.857\\
     \bottomrule
\end{tabular}

==> tables/compare_snufilm_xiph.tex <==
% \begin{tabular}{c|cc|cc|cc|cc}
%     \toprule
%      \multirow{2}{*}{Method} & \multicolumn{2}{c|}{SNUFILM-easy} & \multicolumn{2}{c|}{SNUFILM-medium} & \multicolumn{2}{c|}{SNUFILM-hard}  & \multicolumn{2}{c}{SNUFILM-extreme}\\
%      ~                              & LPIPS    & FID           & LPIPS  & FID      & LPIPS     & FID                   & LPIPS         & FID \\
%      \midrule
%      AMT~\cite{li2023amt}            & 0.022    & 6.139         & 0.035     & 11.039    & 0.060     & 20.810        & 0.112     &   40.075  \\
%      EMA-VFI~\cite{zhang2023ema_vfi} & 0.019    & 5.882         & 0.033     & 11.051    & 0.060    & 20.679        & 0.114     & 39.051 \\
%      URP-Net~\cite{jin2023urpnet}    & 0.018    & 5.669         & 0.034     & 10.983    & 0.062     & 22.127        & 0.112     & 40.098 \\
%      LDMVFI~\cite{danier2024ldmvfi}  & 0.014    & 5.752         & 0.028     & 12.485    & 0.060    & 26.520        & 0.123 & 47.042 \\
%      MADIFF~\cite{huang2024motion}   & 0.013    & 5.334         & 0.027     & 11.022    & 0.058     &22.707        & 0.118  & 44.923    \\
%      CBBD~\cite{lyu2024frame}        & 0.011    & 4.791         & 0.027     & 9.039      & 0.043    & 18.589        & 0.087  & 36.631 \\
%     %eMOMO~\cite{lew2024disentangled} & 0.011    &                  & 0.020     &         & 0.042     &              & 0.087 & \\
%      \textbf{Ours}                   & \textbf{0.010}& \textbf{4.541}& \textbf{0.019}& \textbf{8.499}& \textbf{0.040}& \textbf{15.320}&\textbf{0.084}     &\textbf{27.356}       \\
%      \bottomrule
% \end{tabular}



\begin{tabular}{c|cc|cc|cc|cc|cc|cc}
    \toprule
     \multirow{2}{*}{Method} & \multicolumn{2}{c|}{SNUFILM-easy} & \multicolumn{2}{c|}{SNUFILM-medium} & \multicolumn{2}{c|}{SNUFILM-hard}  & \multicolumn{2}{c|}{SNUFILM-extreme} & \multicolumn{2}{c|}{Xiph-2K} & \multicolumn{2}{c}{Xiph-4K}\\
     ~                              & LPIPS    & FID           & LPIPS      & FID       & LPIPS     & FID           & LPIPS     & FID       &LPIPS  & FID     & LPIPS     & FID\\
     \midrule
     URPNet-Large~\cite{jin2023urpnet}& 0.018    & 5.669        & 0.034     & 10.983    & 0.062     & 22.127        & 0.112     & 40.098    & 0.126   & 14.209     & 0.243    & 32.003   \\
     EMA-VFI~\cite{zhang2023ema_vfi} & 0.019    & 5.882         & 0.033     & 11.051    & 0.060     & 20.679        & 0.114     & 39.051    & 0.107    & 12.332    & 0.233   &  30.675  \\
     AMT-G~\cite{li2023amt}          & 0.022    & 6.139         & 0.035     & 11.039    & 0.060     & 20.810        & 0.112     & 40.075    & 0.109     & 13.089     & 0.209   & 29.512  \\
     SGM-VFI~\cite{liu2024sgm-vfi}   & 0.020    & 7.054         & 0.034     & 12.746    & 0.061     & 22.004        & 0.118     & 41.078    & 0.100    &12.375           &0.216           &28.728    \\
     LDMVFI~\cite{danier2024ldmvfi}  & 0.014    & 5.752         & 0.028     & 12.485    & 0.060     & 26.520        & 0.123     & 47.042    & 0.042    & 11.385      & 0.086    & 21.272 \\
     MADIFF~\cite{huang2024madiff}   & 0.013    & 5.334         & 0.027     & 11.022    & 0.058     &22.707         & 0.118     & 44.923    & -         & -     & -         & -\\
     CBBD~\cite{lyu2024cbbd}        &0.011& 4.791  & 0.027     & 9.039     & 0.043     & 18.589        & 0.087     & 36.631    &  \textbf{0.027}         & 10.168      &  0.063         & 24.621\\
    %eMOMO~\cite{lew2024disentangled} & 0.011    &                  & 0.020     &         & 0.042     &              & 0.087 & \\
     \textbf{Ours}                   & \textbf{0.010}& \textbf{4.541}& \textbf{0.019}& \textbf{8.499}& \textbf{0.040}& \textbf{15.320}&\textbf{0.084} &\textbf{27.356}& 0.029 & \textbf{7.940} &\textbf{0.061} &\textbf{14.132}       \\
     \bottomrule
\end{tabular}


==> tables/compare_training_setting.tex <==
\begin{tabular}{l|cc|cc}
    \toprule
    \multirow{2}{*}{\normalsize stage} & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                      & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    flow loss              &                &                   &               &                      \\
    + image loss           &                &                   &               &                       \\
    + tune auto-encoder    &                &                   &               &                       \\
    \bottomrule
\end{tabular}

==> tables/compare_xiph_psnr_ssim.tex <==
\begin{tabular}{l|cc|cc}
    \toprule
     \multirow{2}{*}{Method}        & \multicolumn{2}{c|}{2K}                & \multicolumn{2}{c}{4K}\\
     ~                              &PSNR                  & SSIM           & PSNR                 & SSIM\\
     \midrule
     URPNet-Large               & 36.455                    & 0.965                 &   33.875                &  0.946         \\
     EMA-VFI                    & 37.128                    & 0.970                 & 34.675                  & 0.948          \\
     AMT-G                      & 36.290                    &  0.965                & 34.550                         &  0.947  \\
     SGM-VFI                    & 36.780                    &  0.968                &  34.227                     & 0.945        \\
     LDMVFI                     & 33.820                    & 0.949                 &    31.390                 & 0.921              \\
     CBBD                       & 35.164                    & 0.958                 &  32.119                  & 0.925                  \\
     {\bf Ours}                 & 35.728                    & 0.958                 &  33.476                   & 0.931             \\
     \bottomrule
\end{tabular}

==> tables/effect_c2f.tex <==
% \begin{tabular}{l|cc|cc|cc}
%          \toprule
%          \multirow{2}{*}{Method} & \multicolumn{2}{c|}{easy} & \multicolumn{2}{c|}{hard}  & \multicolumn{2}{c}{extreme}\\
%          ~                 & LPIPS$\downarrow$    & FID$\downarrow$           & LPIPS$\downarrow$     & FID$\downarrow$           & LPIPS$\downarrow$     & FID$\downarrow$       \\
%          \midrule
%          Full               & 0.0152        & 5.742      & 0.0452   & 17.387     & 0.0943         & 29.198 \\
%          % 1:1:2            & 0.
%          % 1:2:1              & 0.0109        & 4.555     & 0.0199        & 8.452     & 0.0414    & 16.178     &  0.0860       &  28.648             \\
%          % 2:1:1              & 0.0109        & 4.542     & 0.0199        & 8.558     & 0.0415    & 16.432     &  0.0872       &  28.105             \\
%          % 1:1:2              & 0.0109        & 4.555     & 0.0199        & 8.552     & {\bf 0.0400}    & {\bf 14.960}     & {\bf 0.0826}        & {\bf 26.105}             \\
%          % 1:2:1              & 0.0102        & 4.550     & 0.0194        & 8.516     & 0.0407    & 15.563     &  0.0848       & 27.842     \\
%          % 2:1:1              & {\bf 0.0096}  & {\bf 4.538} & {\bf 0.0190}  & {\bf 8.488}     &    0.0414   &    16.178  &   0.0860      &   28.648           \\
%          \textbf{C2F}     & {\bf 0.0098}        & {\bf 4.541}     & {\bf 0.0405}    & {\bf 15.320}     &  {\bf 0.0839}       & {\bf 27.032}          \\   
%          \bottomrule
% \end{tabular}


\begin{tabular}{l|cc|cc}
         \toprule
         \multirow{2}{*}{Method} & \multicolumn{2}{c|}{SNUFILM-hard}  & \multicolumn{2}{c}{SNUFILM-extreme}\\
         ~                 & LPIPS    & FID          & LPIPS     & FID       \\
         \midrule
         Full               & 0.0152        & 5.742      & 0.0943         & 29.198 \\
         % 1:1:2            & 0.
         % 1:2:1              & 0.0109        & 4.555     & 0.0199        & 8.452     & 0.0414    & 16.178     &  0.0860       &  28.648             \\
         % 2:1:1              & 0.0109        & 4.542     & 0.0199        & 8.558     & 0.0415    & 16.432     &  0.0872       &  28.105             \\
         % 1:1:2              & 0.0109        & 4.555     & 0.0199        & 8.552     & {\bf 0.0400}    & {\bf 14.960}     & {\bf 0.0826}        & {\bf 26.105}             \\
         % 1:2:1              & 0.0102        & 4.550     & 0.0194        & 8.516     & 0.0407    & 15.563     &  0.0848       & 27.842     \\
         % 2:1:1              & {\bf 0.0096}  & {\bf 4.538} & {\bf 0.0190}  & {\bf 8.488}     &    0.0414   &    16.178  &   0.0860      &   28.648           \\
         \textbf{C2F}     & {\bf 0.0098}        & {\bf 4.541}      &  {\bf 0.0839}       & {\bf 27.032}          \\   
         \bottomrule
\end{tabular}

==> tables/efficiency_compare_more.tex <==
\begin{tabular}{c|ccccccccc}
    \toprule
    Method   & RIFE     & EBME     & STMFNet & AMT-G    & XVFI   & VFIFormer     & EMA-VFI     & Per-VFI   &  {\bf Ours}     \\
    \midrule
    Runtime &  21.51   &  23.67    & 376.61  & 165.65    & 181.22     &  3270.14  & 557.98     &  450.11  &    198.78            \\
    \bottomrule
\end{tabular}

==> tables/efficiency_compare_v2.tex <==
\begin{tabular}{l|cccc}
    \toprule
    Method  & 256       & 512       & 1024      & 2048      \\   
    \midrule
    LDMVFI    & 8162.47     & 8194.38   & 8315.60   & 9001.63      \\    
    CBBD      & 1766.07     & 1864.01   & 2065.95   & OOM          \\
    \midrule
    \multicolumn{5}{c}{{\bf Ours}} \\
    encoder     & 2.94          & 7.45          &   34.68        & 149.51       \\
    % denoise-8   & 11.39          &  11.44         & 18.11          &  85.69     \\
    % denoise-4   & 11.48          &  18.07         &  85.74         & 368.03       \\
    % denoise-8       &  9.28         &  9.39             &    14.34               & 65.92         \\
    % denoise-4       &  9.36         & 14.32              &    65.97            & 284.69         \\

    denoise-8       &  27.84         &  28.17             &    43.02               & 197.76         \\
    denoise-4       &  28.08         & 42.96              &    197.91            & 854.88         \\
    decoder     & 39.31          & 64.92           & 109.00          & 219.56      \\
    total       & 98.17       & 143.50           & 384.61     &  1421.71      \\

    \bottomrule
    
\end{tabular}

==> tables/performance_autoencoder.tex <==
\begin{tabular}{l|cc|cc}
     \toprule
    \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{SNUFILM-hard}  &  \multicolumn{2}{c}{SNUFILM-extreme} \\
    ~                 & LPIPS          & FID               & LPIPS         & FID                   \\
    \midrule
    2-scale           & 0.0214          & 9.050            & 0.0374        & 17.7105      \\
    3-scale           & 0.0210          & 8.396             & 0.0366        & 17.3926       \\
    4-scale           &                 &                   &               &               \\
    \bottomrule
\end{tabular}

==> tables/rebuttal_main_reuslts.tex <==
\begin{tabular}{l|cc|cc|cc|cc}
         \toprule
         \multirow{2}{*}{Method} & \multicolumn{2}{c|}{easy} & \multicolumn{2}{c|}{medium} & \multicolumn{2}{c|}{hard}  & \multicolumn{2}{c}{extreme}\\
         ~                 & LPIPS    & FID           & LPIPS      & FID       & LPIPS     & FID           & LPIPS     & FID       \\
         \midrule
         \multicolumn{9}{c}{\textit{Evaluation of optical flow}}\\
          GMFlow            & 0.0212        & 6.896     & 0.0348    & 11.356    & 0.0605    & 21.562    & 0.1259    &  47.252     \\    
         Sea-RAFT           & 0.0198      & 6.584     & 0.0362    & 12.903    & 0.0640    & 23.703    & 0.1254    & 45.067       \\
         RAFT               & 0.0185       & 5.429     & 0.0334    & 10.977   & 0.0625     & 22.283    & 0.1199    & 46.414          \\   
         SGM-VFI            & 0.0184         & 5.265     & 0.0317   &  9.846     & 0.0596    & 20.478     &  0.1034       & 38.463          \\
         EMA-VFI            & 0.0165        & 5.060     & 0.0321   &  10.910    & 0.0521    & 19.144     &  0.0968       & 35.346        \\
         \textbf{Ours}      & 0.0098        & 4.541     & 0.0191   &  8.499     & 0.0405    & 15.320     &  0.0839       & 27.032          \\ 
         GT Flow            & {\bf 0.0092}  & {\bf 3.473} & {\bf 0.0139}   &  {\bf 5.622}     & {\bf 0.0264}    & {\bf 11.050}     &  {\bf 0.0424}       & {\bf 20.710}                 \\
         \midrule
         \multicolumn{9}{c}{\textit{Multiscale denoising strategy}}\\
         sep.               & 0.0152        & 5.742      & 0.0278      & 11.489       & 0.0452   & 17.387     & 0.0943         & 29.198 \\
         % 1:1:2            & 0.
         % 1:2:1              & 0.0109        & 4.555     & 0.0199        & 8.452     & 0.0414    & 16.178     &  0.0860       &  28.648             \\
         % 2:1:1              & 0.0109        & 4.542     & 0.0199        & 8.558     & 0.0415    & 16.432     &  0.0872       &  28.105             \\
         1:1:2              & 0.0109        & 4.555     & 0.0199        & 8.552     & {\bf 0.0400}    & {\bf 14.960}     & {\bf 0.0826}        & {\bf 26.105}             \\
         1:2:1              & 0.0102        & 4.550     & 0.0194        & 8.516     & 0.0407    & 15.563     &  0.0848       & 27.842     \\
         2:1:1              & {\bf 0.0096}  & {\bf 4.538} & {\bf 0.0190}  & {\bf 8.488}     &    0.0414   &    16.178  &   0.0860      &   28.648           \\
         \textbf{1:1:1}     & 0.0098        & 4.541     & 0.0191        & 8.499     & 0.0405    & 15.320     &  0.0839       & 27.032          \\ 
         \midrule
         % \multicolumn{9}{c}{\textit{Comparison with more methods}}\\
         % Per-VFI            & 0.0480    & 19.855     &  0.0901      & 34.182    & 0.0399   & 13.467        &  0.0628   & 21.475   \\
         % FILM               & 0.0429    & 16.607     &  0.0889      & 30.002    & 0.0330   & 9.965         &  0.0703   & 17.615  \\        
         % \textbf{Ours}      & {\bf 0.0405}    & {\bf 15.320}     &  {\bf 0.0839}      & {\bf 27.032}    &  {\bf 0.0264}  & {\bf 7.940}         &  {\bf 0.0614}   & {\bf 14.132}     \\  

        \multicolumn{9}{c}{\textit{Comparison with more methods}}\\
         Per-VFI            & 0.0166        & 6.654      & 0.0263   & 11.509     & 0.0480    & 19.855     &  0.0901      & 34.182  \\
         FILM               & 0.0120         & 5.672     & 0.0213   & 8.925        & 0.0429    & 16.607     &  0.0889      & 30.002    \\        
         \textbf{Ours}      & {\bf 0.0098}   & {\bf 4.541}     & {\bf 0.0191}   &  {\bf 8.499}      & {\bf 0.0405}    & {\bf 15.320}     &  {\bf 0.0839}      & {\bf 27.032}     \\   
         \midrule
         \multicolumn{9}{c}{\textit{Different pseudo-labelers}}\\
         GMFlow             & 0.0102        & 4.892     & 0.0212    &  9.135    & {\bf 0.0394}    & {\bf 14.864}      & {\bf 0.0826}     &  {\bf 26.256}     \\        
         Sea-RAFT           & {\bf 0.0096}  & {\bf 4.283} & {\bf 0.0186}   & {\bf 8.067} & 0.0399 & 15.064     &  0.0834      & 27.108          \\
         \textbf{RAFT}      & 0.0098        & 4.541     & 0.0191   &  8.499     & 0.0405    & 15.320     &  0.0839       & 27.032          \\   
         \bottomrule
\end{tabular}

==> tables/runtime_compare.tex <==
% \begin{tabular}{ccccccc}
%     \toprule
%     Method & AMT-G      & SGM-VFI   & LDMVFI    & CBBD     & \bf{Ours-8}    &  \bf{Ours-16}  \\
%     \midrule
%     Timing & 5.58       &           &           &           &  64.76         &   55.24       \\
%     \bottomrule
% \end{tabular}


\begin{tabular}{ccccccc}
    \toprule
    Method      & LDMVFI    & CBBD     & \bf{Ours-8}    &  \bf{Ours-16}  \\
    \midrule
    Timing      &  8601.45  & 1869.44   &  64.76         &   55.24       \\
    \bottomrule
\end{tabular}

==> tables/training_time.tex <==
% \begin{tabular}{ccccc}
%     \toprule
%      Resolution &  Encoder-Decoder      & Diffusion         &  Joint Optimization  & Total\\
%     \midrule
%     128         &  22.37            & 26.42         &  12.34        & 61.13     \\
%     256         &  22.37            & 42.83         &  26.78        & 91.98\\
%     512         &  22.37            & 104.21        &  56.43        & 183.01\\
%     \bottomrule
% \end{tabular}


\begin{tabular}{lccc}
    \toprule
     Stage &  128$\times$128      & 256$\times$256         &  512$\times$512\\
    \midrule
    Encoder-Decoder             &  22.37            & 22.37         &  22.37\\
    Diffusion                   &  {\bf 26.42}           & \underline{42.83}         &  104.21   \\
    Joint Optimization          &  {\bf 12.34}             & \underline{26.78}        &  56.43     \\
    \midrule
    Total                       & {\bf 61.13}             & \underline{91.98}         & 183.02 \\
    \bottomrule
\end{tabular}
